Efficient and Robust Parallel DNN Training through Model Parallelism on Multi-GPU Platform

The training process of Deep Neural Network (DNN) is compute-intensive, often taking days to weeks to train a DNN model. Therefore, parallel execution of DNN training on GPUs is a widely adopted approach to speed up the process nowadays. Due to the implementation simplicity, data parallelism is currently the most commonly used parallelization method. Nonetheless, data parallelism suffers from excessive inter-GPU communication overhead due to frequent weight synchronization among GPUs. Another approach is pipelined model parallelism, which partitions a DNN model among GPUs, and processes multiple mini-batches concurrently. This approach can significantly reduce inter-GPU communication cost compared to data parallelism. However, pipelined model parallelism faces the weight staleness issue; that is, gradients are computed with stale weights, leading to training instability and accuracy loss. In this paper, we present a pipelined model parallel execution method that enables high GPU utilization while maintaining robust training accuracy via a novel weight prediction technique, SpecTrain. Experimental results show that our proposal achieves up to 8.91x speedup compared to data parallelism on a 4-GPU platform while maintaining comparable model accuracy.

==> todo.tex <==
啟中學長覺得要加的敘述
(1) 真實執行下 async. 是不會有 idle 出現的，圖中只是為了清楚表示 weight 版本而做了 alignment，以不影響次序的方式呈現
(2) weight的修正發生在 backward task 做完後，因此 weight version 的分界在於每個 GPU 都做完一個backward之後
